Tailored Visions: Enhancing Text-to-Image Generation with Personalized Prompt Rewriting

Despite significant progress in the field, it is still challenging to create personalized visual representations that align closely with the desires and preferences of individual users. This process requires users to articulate their ideas in words that are both comprehensible to the models and accurately capture their vision, posing difficulties for many users. In this paper, we tackle this challenge by leveraging historical user interactions with the system to enhance user prompts. We propose a novel approach that involves rewriting user prompts based on a newly collected large-scale text-to-image dataset with over 300k prompts from 3115 users. Our rewriting model enhances the expressiveness and alignment of user prompts with their intended visual outputs. Experimental results demonstrate the superiority of our methods over baseline approaches, as evidenced in our new offline evaluation method and online tests. Our code and dataset are available at https://github.com/zzjchen/Tailored-Visions.

==> sec/7_eth_sta.tex <==
\section{Ethics Statement}

In this section, we discuss three primary ethical considerations regarding both our PIP dataset and the proposed method.

\begin{itemize}%[topsep=3pt, itemsep=2pt, parsep=0pt, leftmargin=10pt]
  \item \textbf{Copyright.}
  When using our text-to-image generation website, all users consent to our privacy policy and data usage agreement.
  This includes academic utilization and the dissemination of any content hosted on the server, such as anonymized prompts, images, and user iterations.

  \item \textbf{Privacy.}
  We've ensured that all user data in the PIP dataset, including usernames and other private details, has been anonymized.
  It is worth noting that while rare, there is a possibility that certain prompts could contain sensitive information. But, this is uncommon because our website has strict rules against writing personal information in the prompts, and has professional detectors to eliminate any violative content as well.
  \item \textbf{Potential Harm.}
  Although we have built strong detectors to filter out inappropriate material on our website, there remains a potential for occasional instances of NSFW (Not Safe for Work) content to emerge in PIP dataset.
  %Furthermore, even with the inclusion of a safety module, it's possible for Stable Diffusion v1-5 to occasionally produce content that could be considered potentially unsafe.
  Furthermore, our method uses Stable Diffusion v1-5 and ChatGPT as a prior, therefore it inherits any problematic biases and limitations that they may have.
\end{itemize}
